Interpretable CNN-Multilevel Attention Transformer for Rapid Recognition of Pneumonia from Chest X-Ray Images

Chest imaging plays an essential role in diagnosing and predicting patients with COVID-19 with evidence of worsening respiratory status. Many deep learning-based approaches for pneumonia recognition have been developed to enable computer-aided diagnosis. However, the long training and inference time makes them inflexible, and the lack of interpretability reduces their credibility in clinical medical practice. This paper aims to develop a pneumonia recognition framework with interpretability, which can understand the complex relationship between lung features and related diseases in chest X-ray (CXR) images to provide high-speed analytics support for medical practice. To reduce the computational complexity to accelerate the recognition process, a novel multi-level self-attention mechanism within Transformer has been proposed to accelerate convergence and emphasize the task-related feature regions. Moreover, a practical CXR image data augmentation has been adopted to address the scarcity of medical image data problems to boost the model's performance. The effectiveness of the proposed method has been demonstrated on the classic COVID-19 recognition task using the widespread pneumonia CXR image dataset. In addition, abundant ablation experiments validate the effectiveness and necessity of all of the components of the proposed method.

==> table_dp_exp.tex <==
\begin{table}[tb]
  \centering
  \resizebox{.9\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c}
    \toprule
    \sc Method & \sc Differential Privacy & MTARSI & MSTAR & FGSCR-42 & Aircraft-16 \\
    \midrule
    \multirow{5}[2]{*}{\sc FedAvg} & \textit{wo}  &  57.55$_{\pm 1.03}$  &  47.56$_{\pm 0.74}$  & 65.15$_{\pm 2.11}$  &  54.08$_{\pm 1.83}$\\
       & \textit{w} ($\tau=1e^{-3}$) &  56.21$_{\pm 0.72}$  &  45.97$_{\pm 0.12}$  &  64.21$_{\pm 1.16}$  & 53.31$_{\pm 0.46}$ \\
       & \textit{w} ($\tau=1e^{-2}$) &  54.64$_{\pm 0.44}$  &  42.30$_{\pm 0.34}$  &  62.77$_{\pm 0.63}$  & 50.56$_{\pm 0.51}$ \\
       & \textit{w} ($\tau=5e^{-2}$) &  47.21$_{\pm 0.21}$  &  38.22$_{\pm 0.93}$  &  52.99$_{\pm 0.46}$  & 43.53$_{\pm 0.78}$ \\
        & \cellcolor{green! 20} Mean Variation &  \cellcolor{green! 20} 8.45 $\downarrow$  &  \cellcolor{green! 20} 11.33 $\downarrow$ & \cellcolor{green! 20} 7.93 $\downarrow$   &  \cellcolor{green! 20} 9.15 $\downarrow$\\
    \midrule
      \multirow{5}[2]{*}{\sc FedBN} &  \textit{wo}  &  73.51$_{\pm 1.04}$  & 66.13$_{\pm 0.06}$  &  81.93$_{\pm 1.12}$  & 61.92$_{\pm 1.81}$ \\
       & \textit{w} ($\tau=1e^{-3}$) &  69.52$_{\pm 0.23}$  &  62.70$_{\pm 0.36}$  &  77.43$_{\pm 0.06}$  & 58.62$_{\pm 1.71}$ \\
       & \textit{w} ($\tau=1e^{-2}$) &  67.98$_{\pm 0.48}$  &  61.07$_{\pm 0.52}$  &  75.75$_{\pm 1.03}$  & 57.25$_{\pm 1.67}$ \\
       & \textit{w} ($\tau=5e^{-2}$) &  65.33$_{\pm 1.80}$  &  58.06$_{\pm 0.02}$  &  73.10$_{\pm 0.45}$  & 55.47$_{\pm 1.61}$ \\
       & \cellcolor{green! 20} Mean Variation &  \cellcolor{green! 20} 4.18 $\downarrow$  &  \cellcolor{green! 20} 4.07 $\downarrow$  &  \cellcolor{green! 20} 4.83 $\downarrow$  & \cellcolor{green! 20} 3.45 $\downarrow$  \\
    \midrule
       \multirow{5}[2]{*}{\sc PerFedAvg} &  \textit{wo}  &  78.30$_{\pm 0.47}$  &  86.31$_{\pm 0.54}$  &  75.95$_{\pm 1.28}$  & 69.01$_{\pm 1.29}$ \\
       & \textit{w} ($\tau=1e^{-3}$) &  76.34$_{\pm 0.55}$  &  84.15$_{\pm 0.73}$  &  74.05$_{\pm 1.92}$  & 67.28$_{\pm 1.26}$ \\
       & \textit{w} ($\tau=1e^{-2}$) &  73.61$_{\pm 0.31}$  &  81.09$_{\pm 0.81}$  &  71.37$_{\pm 1.00}$  & 64.87$_{\pm 0.21}$ \\
       & \textit{w} ($\tau=5e^{-2}$) &  71.62$_{\pm 0.49}$  &  78.60$_{\pm 0.29}$  &  69.51$_{\pm 0.75}$  & 63.11$_{\pm 0.18}$ \\
       & \cellcolor{green! 20} Mean Variation & \cellcolor{green! 20} \underline{3.45} $\downarrow$  &  \cellcolor{green! 20} \underline{3.95} $\downarrow$  &  \cellcolor{green! 20} \underline{3.21} $\downarrow$  &  \cellcolor{green! 20} \underline{2.95} $\downarrow$  \\
    \midrule
      \multirow{5}[2]{*}{\sc FedBE} &  \textit{wo}  &  85.10$_{\pm 0.22}$  & 88.94$_{\pm 0.41}$   &  78.45$_{\pm 1.10}$  & 79.62$_{\pm 0.75}$ \\
       & \textit{w} ($\tau=1e^{-3}$) &  82.97$_{\pm 0.09}$  &  86.71$_{\pm 0.29}$  &  76.49$_{\pm 0.25}$  & 77.62$_{\pm 0.23}$ \\
       & \textit{w} ($\tau=1e^{-2}$) &  80.85$_{\pm 0.26}$  &  84.49$_{\pm 0.38}$  &  74.53$_{\pm 0.60}$  & 75.64$_{\pm 0.51}$ \\
       & \textit{w} ($\tau=5e^{-2}$) &  77.82$_{\pm 0.82}$  &  81.44$_{\pm 0.66}$  &  71.78$_{\pm 1.01}$  & 72.89$_{\pm 0.49}$ \\
       & \cellcolor{green! 20} Mean Variation &  \cellcolor{green! 20} 4.42 $\downarrow$ &  \cellcolor{green! 20} 4.62 $\downarrow$ &  \cellcolor{green! 20} 4.17 $\downarrow$ &  \cellcolor{green! 20} 4.14 $\downarrow$\\
    \midrule
    \multirow{5}[2]{*}{\sc \bf PRFL (Ours)} &  \textit{wo} &  90.35$_{\pm 0.42}$  &  97.18$_{\pm 0.15}$  & 84.49$_{\pm 0.91}$  &  87.04$_{\pm 0.80}$ \\
       & \textit{w} ($\tau=1e^{-3}$) &  89.46$_{\pm 0.48}$  &  96.21$_{\pm 0.99}$  &  83.65$_{\pm 0.40}$  &  86.17$_{\pm 0.56}$ \\
       & \textit{w} ($\tau=1e^{-2}$) &  88.71$_{\pm 0.77}$  &  94.89$_{\pm 0.17}$  &  82.33$_{\pm 0.59}$  &  84.98$_{\pm 0.55}$ \\
       & \textit{w} ($\tau=5e^{-2}$) &  86.33$_{\pm 0.75}$  &  92.73$_{\pm 0.38}$  &  80.27$_{\pm 0.27}$  &  82.87$_{\pm 0.23}$ \\
       & \cellcolor{red! 20} Mean Variation &  \cellcolor{red! 20} \bf 2.01 $\downarrow$ &  \cellcolor{red! 20} \bf 2.15 $\downarrow$ &  \cellcolor{red! 20} \bf 2.22 $\downarrow$ &  \cellcolor{red! 20} \bf 2.17 $\downarrow$\\
    \bottomrule
    \end{tabular}}
    \caption{Results of Differential Privacy experiments (DP factor $\tau \in \{1e^{-3}, 1e^{-2}, 5e^{-2}\}$) of the proposed PRFL and baseline methods under four fine-grained classification datasets under the Dirichlet Non-IID setting ($\lambda=0.1$), where \textbf{Bold} denotes the optimal result, \underline{Underline} denotes the suboptimal result, $\downarrow$ denotes the degradation of the performance, with lower being better. Note that \textit{w} and \textit{wo} present \textit{with} and \textit{without}, respectively.}
  \label{tab:dpexp}
\end{table}%
